Stabilizer Reduction for Derived Stacks and Applications to Sheaf-Theoretic Invariants

We construct a canonical stabilizer reduction $\widetilde{X}$ for any derived $1$-algebraic stack $X$ over $\mathbb{C}$ as a sequence of derived Kirwan blow-ups, under mild natural conditions that include the existence of a good moduli space for the classical truncation $X_{\mathrm{cl}}$. Our construction has several desired features: it naturally generalizes Kirwan's classical partial desingularization algorithm to the context of derived algebraic geometry, preserves quasi-smoothness, and is a derived enhancement of the intrinsic stabilizer reduction constructed by Kiem, Li and the third author. Moreover, if $X$ is $(-1)$-shifted symplectic, we show that the semi-perfect and almost perfect obstruction theory of $\widetilde{X}_{\mathrm{cl}}$ and the associated virtual fundamental cycle and virtual structure sheaf, constructed by the same authors, are naturally induced by $\widetilde{X}$ and its derived tangent complex. As corollaries, we define virtual classes for moduli stacks of semistable sheaves on surfaces, give a fully derived perspective on generalized Donaldson-Thomas invariants of Calabi-Yau threefolds and define new generalized Vafa-Witten invariants for surfaces via Kirwan blow-ups.

==> moremacros.tex <==
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{sublem}[thm]{Sublemma}
\newtheorem{defi}[thm]{Definition}
\newtheorem{rmk}[thm]{Remark}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop-defi}[thm]{Proposition-Definition}
\newtheorem{thm-defi}[thm]{Theorem-Definition}
\newtheorem{lem-defi}[thm]{Lemma-Definition}
\newtheorem{assum}[thm]{Assumption}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{exam}[thm]{Example}
\newtheorem{hyp}[thm]{Hypothesis}
\newtheorem{setup}[thm]{Setup}
\newtheorem{setup-def}[thm]{Setup-Definition}
\newtheorem{notation}[thm]{Notation}
\newtheorem{question}[thm]{Question}
\newtheorem{goal}[thm]{Goal}



\newenvironment{sproof}{%
  \renewcommand{\proofname}{Proof sketch}\proof}{\endproof}

\newdimen\argwidth
\def\db[#1\db]{
 \setbox0=\hbox{$#1$}\argwidth=\wd0
 \setbox0=\hbox{$\left[\box0\right]$}
  \advance\argwidth by -\wd0
 \left[\kern.3\argwidth\box0 \kern.3\argwidth\right]}


\newcommand{\aA}{\mathcal{A}}
\newcommand{\bB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\dD}{\mathcal{D}}
\newcommand{\eE}{\mathcal{E}}
\newcommand{\fF}{\mathcal{F}}
\newcommand{\gG}{\mathcal{G}}
\newcommand{\hH}{\mathcal{H}}
\newcommand{\iI}{\mathcal{I}}
\newcommand{\jJ}{\mathcal{J}}
\newcommand{\kK}{\mathcal{K}}
\newcommand{\lL}{\mathcal{L}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\nN}{\mathcal{N}}
\newcommand{\oO}{\mathcal{O}}
\newcommand{\pP}{\mathcal{P}}
\newcommand{\qQ}{\mathcal{Q}}
\newcommand{\rR}{\mathcal{R}}
\newcommand{\sS}{\mathcal{S}}
\newcommand{\tT}{\mathcal{T}}
\newcommand{\uU}{\mathcal{U}}
\newcommand{\vV}{\mathcal{V}}
\newcommand{\wW}{\mathcal{W}}
\newcommand{\xX}{\mathcal{X}}
\newcommand{\yY}{\mathcal{Y}}
\newcommand{\zZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbb{A}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bT}{\mathbb{T}}

\newcommand{\fm}{\mathfrak{m}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fr}{\mathfrak{r}}
\newcommand{\fh}{\mathfrak{h}}
\newcommand{\fc}{\mathfrak{c}}

\renewcommand{\tilde}{\widetilde}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tW}{\tilde{W}}

%\newcommand{\Ob}{\mathcal{O}b}
\newcommand{\OB}{\mathop{\rm Ob}\nolimits}
\newcommand{\Hone}{\mathop{H^1}\nolimits}

\newcommand{\defeq}{\mathrel{\mathop:}=}

\renewcommand{\hat}{\widehat}
\newcommand{\wH}{\widehat{H}}
\newcommand{\tom}{\tilde{\omega}}
\newcommand{\hatom}{\hat{\omega}}
\newcommand{\bom}{\bar{\omega}}
%\newcommand{\coker}{\mathop{\rm coker}\nolimits}
\newcommand{\dspec}{\mathop{\mathbf{Spec}}\nolimits}
\newcommand{\lr}{\longrightarrow}
\newcommand{\Hom}{\mathop{\rm Hom}\nolimits}
%\newcommand{\id}{\textrm{id}}
\newcommand{\Ext}{\mathop{\rm Ext}\nolimits}
%\newcommand{\Spec}{\mathop{\rm Spec}\nolimits}
%\newcommand{\Coh}{\mathop{\rm Coh}\nolimits}
\newcommand{\im}{\mathop{\rm im}\nolimits}
\newcommand{\Crit}{\mathop{\rm Crit}\nolimits}
\newcommand{\Ker}{\mathop{\rm Ker}\nolimits}
%\newcommand{\GL}{\mathop{\rm GL}\nolimits}
%\newcommand{\PGL}{\mathop{\rm PGL}\nolimits}


\def\Abul{A^\bullet}
\def\ck{\mathrm{ck}}
\def\fR{\mathfrak{R}}
\def\blue{\color{blue}}
\def\lal{_\lambda}
\def\lra{\longrightarrow}
\def\ti{\tilde}
\def\defeq{=:}
\def\bl{\bigl(} \def\br{\bigr)}
\def\sO{\mathscr O}
\def\CC{\mathbb C}
\def\sta{^\ast}
%\def\red{\color{red}}
\def\lalp{_\alpha}
\def\sub{\subset}
\def\cM{\mM}
\def\tcM{\tilde\cM}
\def\virt{^{\mathrm{vir}}}
\def\upmo{^{-1}}
\def\lbe{_\beta}
\def\hatom{\hat\omega}
\def\hW{\hat W}
\def\uss{^{ss}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}

\def\git{/\!\!/}
\def\lalp{_\alpha }
\def\lab{_{\alpha\beta}}
\def\lbet{_\beta}
\def\mapright#1{\,\smash{\mathop{\lra}\limits^{#1}}\,}
\def\rred{{\mathrm{red}}}
\def\hV{\hat V}
\def\hU{\hat U}
\def\uss{^{ss}}
\def\us{^s}
\def\cE{{\mathcal E}}

% Letters
\newcommand{\TT}{\mathbf{T}}
\newcommand{\BA}{{\mathbb{A}}}
\newcommand{\BB}{{\mathbb{B}}}
\newcommand{\BC}{{\mathbb{C}}}
\newcommand{\BD}{{\mathbb{D}}}
\newcommand{\BE}{{\mathbb{E}}}
\newcommand{\BF}{{\mathbb{F}}}
\newcommand{\BG}{{\mathbb{G}}}
\newcommand{\BH}{{\mathbb{H}}}
\newcommand{\BI}{{\mathbb{I}}}
\newcommand{\BJ}{{\mathbb{J}}}
\newcommand{\BK}{{\mathbb{K}}}
\newcommand{\BL}{{\mathbb{L}}}
\newcommand{\BM}{{\mathbb{M}}}
\newcommand{\BN}{{\mathbb{N}}}
\newcommand{\BO}{{\mathbb{O}}}
\newcommand{\BP}{{\mathbb{P}}}
\newcommand{\BQ}{{\mathbb{Q}}}
\newcommand{\BR}{{\mathbb{R}}}
\newcommand{\BS}{{\mathbb{S}}}
\newcommand{\BT}{{\mathbb{T}}}
\newcommand{\BU}{{\mathbb{U}}}
\newcommand{\BV}{{\mathbb{V}}}
\newcommand{\BW}{{\mathbb{W}}}
\newcommand{\BX}{{\mathbb{X}}}
\newcommand{\BY}{{\mathbb{Y}}}
\newcommand{\BZ}{{\mathbb{Z}}}

\newcommand{\CA}{{\mathcal A}}
\newcommand{\CB}{{\mathcal B}}
%\newcommand{\CC}{{\mathcal C}}
%\newcommand{\CD}{{\mathcal D}}
\newcommand{\CE}{{\mathcal E}}
\newcommand{\CF}{{\mathcal F}}
\newcommand{\CG}{{\mathcal G}}
\newcommand{\CH}{{\mathcal H}}
\newcommand{\CI}{{\mathcal I}}
\newcommand{\CJ}{{\mathcal J}}
\newcommand{\CK}{{\mathcal K}}
\newcommand{\CL}{{\mathcal L}}
\newcommand{\CM}{{\mathcal M}}
\newcommand{\CN}{{\mathcal N}}
\newcommand{\CO}{{\mathcal O}}
\newcommand{\CP}{{\mathcal P}}
\newcommand{\CQ}{{\mathcal Q}}
\newcommand{\CR}{{\mathcal R}}
\newcommand{\CS}{{\mathcal S}}
\newcommand{\CT}{{\mathcal T}}
\newcommand{\CU}{{\mathcal U}}
\newcommand{\CV}{{\mathcal V}}
\newcommand{\CW}{{\mathcal W}}
\newcommand{\CX}{{\mathcal X}}
\newcommand{\CY}{{\mathcal Y}}
\newcommand{\CZ}{{\mathcal Z}}

\newcommand{\simto}{\,\widetilde{\to}\,}
\newcommand{\into}{\hookrightarrow}
\newcommand{\onto}{\twoheadrightarrow}
\newcommand{\Hess}{\mathsf{Hess}}
\newcommand{\BRcrit}{\mathbb{R}\mathrm{crit}}
\newcommand{\derived}{\mathbf{D}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\RR}{\mathbf R}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\Bl}{\operatorname{Bl}}
\newcommand{\Tot}{\operatorname{Tot}}
\newcommand{\Mbar}{{\overline M}}
\newcommand{\Pic}{\mathop{\rm Pic}\nolimits}
\newcommand{\PT}{\mathsf{PT}}
\newcommand{\DT}{\mathsf{DT}}
\newcommand{\GW}{\mathsf{GW}}
\newcommand{\Q}{\mathsf{Q}}
\newcommand{\ch}{\mathsf{ch}}
\newcommand{\HH}{\mathrm{H}}
\newcommand{\OO}{\mathscr O}
\newcommand{\Fram}{\mathsf{Fr}}
\newcommand{\crit}{\operatorname{crit}}
\newcommand{\zetass}{\zeta\textrm{-ss}}
\newcommand{\zetast}{\zeta\textrm{-st}}
%\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     %\hbox{\scriptsize.}\hbox{\scriptsize.}}}=}


\DeclareMathOperator{\Hilb}{Hilb}
\DeclareMathOperator{\Quot}{Quot}
\DeclareMathOperator{\Chow}{Chow}
\DeclareMathOperator{\NCHilb}{ncHilb}
\DeclareMathOperator{\NCQuot}{ncQuot}
\DeclareMathOperator{\Sets}{Sets}
\DeclareMathOperator{\Sch}{Sch}
\DeclareMathOperator{\coh}{coh}
\DeclareMathOperator{\Coh}{Coh}
\DeclareMathOperator{\QCoh}{QCoh}
\DeclareMathOperator{\red}{red}
\DeclareMathOperator{\Der}{Der}
\DeclareMathOperator{\der}{der}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Mod}{Mod}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\ob}{ob}
\DeclareMathOperator{\Ob}{Ob}
\DeclareMathOperator{\Rep}{Rep}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\PGL}{PGL}
\DeclareMathOperator{\Mat}{Mat}
\DeclareMathOperator{\op}{op}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\vir}{\mathrm{vir}}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\Perf}{Perf}
\DeclareMathOperator{\bounded}{b}
\DeclareMathOperator{\colim}{colim}
\DeclareMathOperator{\Def}{Def}
\DeclareMathOperator{\Jac}{Jac}
\DeclareMathOperator{\pr}{pr}
\DeclareMathOperator{\At}{At}

\renewcommand{\ss}{\operatorname{ss}}

%%%%%%%%% Michail's commands %%%%%%%%
%\newcommand{\fg}{{\mathfrak g}}
%\newcommand{\fm}{{\mathfrak m}}
%\newcommand{\lr}{\longrightarrow}
\newcommand{\bfa}{{\mathbf a}}
\newcommand{\unal}{\underline{\alpha}}
\newcommand{\unbet}{\underline{\beta}}
\newcommand{\ungam}{\underline{\gamma}}
\renewcommand{\hat}{\widehat}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\gl}{\mathfrak{gl}}
\newcommand{\cdga}{{\mathrm{cdga_{\BC}^{\leq 0}}}}
\newcommand{\dga}{\mathrm{dga}_\BC}
\newcommand{\boldit}[1]{\boldsymbol{#1}}
\DeclareMathAlphabet\BCal{OMS}{cmsy}{b}{n}
\newcommand{\cC}{{\mathcal C}}
